A resampling approach for causal inference on novel two-point time-series with application to identify risk factors for type-2 diabetes and cardiovascular disease

Two-point time-series data, characterized by baseline and follow-up observations, are frequently encountered in health research. We study a novel two-point time series structure without a control group, which is driven by an observational routine clinical dataset collected to monitor key risk markers of type-$2$ diabetes (T2D) and cardiovascular disease (CVD). We propose a resampling approach called 'I-Rand' for independently sampling one of the two time points for each individual and making inference on the estimated causal effects based on matching methods. The proposed method is illustrated with data from a service-based dietary intervention to promote a low-carbohydrate diet (LCD), designed to impact risk of T2D and CVD. Baseline data contain a pre-intervention health record of study participants, and health data after LCD intervention are recorded at the follow-up visit, providing a two-point time-series pattern without a parallel control group. Using this approach we find that obesity is a significant risk factor of T2D and CVD, and an LCD approach can significantly mitigate the risks of T2D and CVD. We provide code that implements our method.

==> Statistics in Medicine/files/tables/description.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
  &        &  count &        mean &        std &      min &         25\% &         50\% &         75\% &         max \\
State & Variable &        &             &            &          &             &             &             &             \\
\midrule
  & Gender &  256.0 &    0.589844 &   0.492825 &    0.000 &    0.000000 &    1.000000 &    1.000000 &    1.000000 \\
  & Age &  256.0 &   61.574219 &  12.110697 &   23.000 &   53.000000 &   60.000000 &   71.000000 &   91.000000 \\
  & State &  256.0 &    0.000000 &   0.000000 &    0.000 &    0.000000 &    0.000000 &    0.000000 &    0.000000 \\
  & Height &   75.0 &    1.706027 &   0.092245 &    1.473 &    1.625000 &    1.720000 &    1.770000 &    1.900000 \\
  & Weight &  251.0 &   96.159761 &  18.621362 &   55.300 &   83.700000 &   95.000000 &  107.000000 &  159.000000 \\
  & BMI &   66.0 &   33.887432 &   6.070832 &   21.660 &   29.890000 &   33.495000 &   36.980000 &   57.100000 \\
  & Diabetes &  256.0 &    1.281250 &   0.811075 &    0.000 &    1.000000 &    2.000000 &    2.000000 &    2.000000 \\
  & HbA1c/   mmol/mol &  202.0 &   61.376238 &  20.651986 &   37.000 &   45.000000 &   54.500000 &   71.000000 &  135.000000 \\
  & Gamma-G.T Level/   U/L &  137.0 &   78.664234 &  78.426181 &   14.000 &   35.000000 &   51.000000 &   95.000000 &  489.000000 \\
0  & Serum Cholesterol &  176.0 &    5.313693 &   1.302405 &    2.500 &    4.385000 &    5.200000 &    6.225000 &    9.300000 \\
  & HDL Cholesterol &  195.0 &    1.280256 &   0.421051 &    0.600 &    1.000000 &    1.200000 &    1.450000 &    3.500000 \\
  & Cholesterol Ratio &  157.0 &    4.304968 &   1.361320 &    1.200 &    3.000000 &    4.000000 &    5.000000 &    8.830000 \\
  & Triglyceride &  143.0 &    2.409650 &   1.445505 &    0.700 &    1.435000 &    2.000000 &    2.990000 &    7.910000 \\
  & Triglyceride/HDL Ratio &   80.0 &    2.203694 &   1.673170 &    0.400 &    1.087413 &    1.714407 &    2.753598 &    8.777778 \\
  & Systolic &  171.0 &  143.502924 &  15.476500 &  114.000 &  132.000000 &  142.000000 &  152.000000 &  223.000000 \\
  & Diastolic &  171.0 &   84.163743 &  10.320572 &   65.000 &   78.000000 &   80.000000 &   90.000000 &  122.000000 \\
  & TSH &   26.0 &    2.400000 &   1.398451 &    0.020 &    1.202500 &    2.375000 &    3.220000 &    5.050000 \\
  & T4 &   25.0 &   15.004000 &   2.793665 &    9.700 &   13.400000 &   14.500000 &   16.000000 &   22.900000 \\
  & HB &   22.0 &  145.136364 &   8.741229 &  123.000 &  140.250000 &  146.000000 &  150.500000 &  159.000000 \\
  & HMCT &   22.0 &    0.438636 &   0.026058 &    0.380 &    0.422500 &    0.440000 &    0.450000 &    0.500000 \\
  & months &  256.0 &    0.000000 &   0.000000 &    0.000 &    0.000000 &    0.000000 &    0.000000 &    0.000000 \\
  \midrule
  & Gender &  256.0 &    0.589844 &   0.492825 &    0.000 &    0.000000 &    1.000000 &    1.000000 &    1.000000 \\
  & Age &  256.0 &   61.574219 &  12.110697 &   23.000 &   53.000000 &   60.000000 &   71.000000 &   91.000000 \\
  & State &  256.0 &    1.000000 &   0.000000 &    1.000 &    1.000000 &    1.000000 &    1.000000 &    1.000000 \\
  & Height &   75.0 &    1.706027 &   0.092245 &    1.473 &    1.625000 &    1.720000 &    1.770000 &    1.900000 \\
  & Weight &  251.0 &   87.070120 &  17.351535 &   51.000 &   75.000000 &   84.400000 &   97.100000 &  140.000000 \\
  & BMI &   65.0 &   30.356462 &   5.922518 &   19.240 &   27.040000 &   29.270000 &   32.470000 &   53.620000 \\
  & Diabetes &  256.0 &    0.718750 &   0.867157 &    0.000 &    0.000000 &    0.000000 &    2.000000 &    2.000000 \\
  & HbA1c/   mmol/mol &  201.0 &   45.925373 &   9.318766 &   32.000 &   40.000000 &   43.000000 &   50.000000 &   84.000000 \\
  & Gamma-G.T Level/   U/L &  137.0 &   44.660584 &  39.049598 &    7.000 &   22.000000 &   32.000000 &   52.000000 &  260.000000 \\
1  & Serum Cholesterol &  174.0 &    4.892414 &   1.246772 &    2.400 &    4.025000 &    4.700000 &    5.700000 &    8.800000 \\
  & HDL Cholesterol &  189.0 &    1.412751 &   0.542463 &    0.700 &    1.090000 &    1.340000 &    1.610000 &    4.900000 \\
  & Cholesterol Ratio &  156.0 &    3.756667 &   1.073727 &    1.350 &    3.000000 &    3.775000 &    4.420000 &    7.000000 \\
  & Triglyceride &  132.0 &    1.522576 &   0.887664 &    0.560 &    0.930000 &    1.300000 &    1.795000 &    6.200000 \\
  & Triglyceride/HDL Ratio &   71.0 &    1.221976 &   0.935913 &    0.150 &    0.664018 &    0.963636 &    1.398688 &    5.777778 \\
  & Systolic &  170.0 &  132.100000 &  11.020503 &  108.000 &  125.000000 &  132.000000 &  139.500000 &  170.000000 \\
  & Diastolic &  170.0 &   77.794118 &   7.569713 &   54.000 &   71.250000 &   78.000000 &   82.000000 &  110.000000 \\
  & TSH &   26.0 &    1.919231 &   1.056757 &    0.140 &    0.855000 &    1.975000 &    2.720000 &    3.790000 \\
  & T4 &   25.0 &   15.480000 &   2.238675 &   11.400 &   13.900000 &   15.200000 &   16.200000 &   20.800000 \\
  & HB &   22.0 &  141.636364 &  10.513236 &  115.000 &  137.000000 &  142.000000 &  146.750000 &  161.000000 \\
  & HMCT &   22.0 &    0.421364 &   0.031517 &    0.330 &    0.410000 &    0.425000 &    0.440000 &    0.480000 \\
  & months &  256.0 &   22.199219 &  17.456370 &    1.000 &    8.000000 &   19.000000 &   32.000000 &   84.000000 \\
\bottomrule
\end{tabular}


==> Statistics in Medicine/files/tables/summary.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
  &        &  count &     mean &     std &      min &      25\% &      50\% &      75\% &      max \\
LCD & Variable &        &          &         &          &          &          &          &          \\
\midrule
  & Gender &    256 &    0.590 &   0.493 &    0.000 &    0.000 &    1.000 &    1.000 &    1.000 \\
  & Age &    256 &   61.574 &  12.111 &   23.000 &   53.000 &   60.000 &   71.000 &   91.000 \\
  & Height &     75 &    1.706 &   0.092 &    1.473 &    1.625 &    1.720 &    1.770 &    1.900 \\
  & Weight &    251 &   96.160 &  18.621 &   55.300 &   83.700 &   95.000 &  107.000 &  159.000 \\
  & BMI &     66 &   33.887 &   6.071 &   21.660 &   29.890 &   33.495 &   36.980 &   57.100 \\
0  & T2D &    256 &    1.281 &   0.811 &    0.000 &    1.000 &    2.000 &    2.000 &    2.000 \\
  & HbA1c/   mmol/mol &    202 &   61.376 &  20.652 &   37.000 &   45.000 &   54.500 &   71.000 &  135.000 \\
%  & Gamma-G.T Level/   U/L &    137 &   78.664 &  78.426 &   14.000 &   35.000 &   51.000 &   95.000 &  489.000 \\
  & TBC &    176 &    5.314 &   1.302 &    2.500 &    4.385 &    5.200 &    6.225 &    9.300 \\
 & HDL &    195 &    1.280 &   0.421 &    0.600 &    1.000 &    1.200 &    1.450 &    3.500 \\
%  & Cholesterol Ratio &    157 &    4.305 &   1.361 &    1.200 &    3.000 &    4.000 &    5.000 &    8.830 \\
%  & Triglyceride &    143 &    2.410 &   1.446 &    0.700 &    1.435 &    2.000 &    2.990 &    7.910 \\
%  & Triglyceride/HDL Ratio &     80 &    2.204 &   1.673 &    0.400 &    1.087 &    1.714 &    2.754 &    8.778 \\
  & SBP &    171 &  143.503 &  15.476 &  114.000 &  132.000 &  142.000 &  152.000 &  223.000 \\
%  & Diastolic &    171 &   84.164 &  10.321 &   65.000 &   78.000 &   80.000 &   90.000 &  122.000 \\
%  & TSH &     26 &    2.400 &   1.398 &    0.020 &    1.202 &    2.375 &    3.220 &    5.050 \\
%  & T4 &     25 &   15.004 &   2.794 &    9.700 &   13.400 &   14.500 &   16.000 &   22.900 \\
%  & HB &     22 &  145.136 &   8.741 &  123.000 &  140.250 &  146.000 &  150.500 &  159.000 \\
%  & HMCT &     22 &    0.439 &   0.026 &    0.380 &    0.422 &    0.440 &    0.450 &    0.500 \\
%  & months &    256 &    0.000 &   0.000 &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 \\
  \midrule
  & Gender &    256 &    0.590 &   0.493 &    0.000 &    0.000 &    1.000 &    1.000 &    1.000 \\
  & Age &    256 &   63.424 &  12.387 &   23.167 &   54.750 &   62.750 &   73.500 &   91.500 \\
  & Height &     75 &    1.706 &   0.092 &    1.473 &    1.625 &    1.720 &    1.770 &    1.900 \\
  & Weight &    251 &   87.070 &  17.352 &   51.000 &   75.000 &   84.400 &   97.100 &  140.000 \\
  & BMI &     65 &   30.356 &   5.923 &   19.240 &   27.040 &   29.270 &   32.470 &   53.620 \\
1  & T2D &    256 &    0.719 &   0.867 &    0.000 &    0.000 &    0.000 &    2.000 &    2.000 \\
  & HbA1c/   mmol/mol &    201 &   45.925 &   9.319 &   32.000 &   40.000 &   43.000 &   50.000 &   84.000 \\
%  & Gamma-G.T Level/   U/L &    137 &   44.661 &  39.050 &    7.000 &   22.000 &   32.000 &   52.000 &  260.000 \\
  & TBC &    174 &    4.892 &   1.247 &    2.400 &    4.025 &    4.700 &    5.700 &    8.800 \\
 & HDL &    189 &    1.413 &   0.542 &    0.700 &    1.090 &    1.340 &    1.610 &    4.900 \\
%  & Cholesterol Ratio &    156 &    3.757 &   1.074 &    1.350 &    3.000 &    3.775 &    4.420 &    7.000 \\
%  & Triglyceride &    132 &    1.523 &   0.888 &    0.560 &    0.930 &    1.300 &    1.795 &    6.200 \\
%  & Triglyceride/HDL Ratio &     71 &    1.222 &   0.936 &    0.150 &    0.664 &    0.964 &    1.399 &    5.778 \\
  & SBP &    170 &  132.100 &  11.021 &  108.000 &  125.000 &  132.000 &  139.500 &  170.000 \\
%  & Diastolic &    170 &   77.794 &   7.570 &   54.000 &   71.250 &   78.000 &   82.000 &  110.000 \\
%  & TSH &     26 &    1.919 &   1.057 &    0.140 &    0.855 &    1.975 &    2.720 &    3.790 \\
%  & T4 &     25 &   15.480 &   2.239 &   11.400 &   13.900 &   15.200 &   16.200 &   20.800 \\
%  & HB &     22 &  141.636 &  10.513 &  115.000 &  137.000 &  142.000 &  146.750 &  161.000 \\
%  & HMCT &     22 &    0.421 &   0.032 &    0.330 &    0.410 &    0.425 &    0.440 &    0.480 \\
  & months &    256 &   22.199 &  17.456 &    1.000 &    8.000 &   19.000 &   32.000 &   84.000 \\
\bottomrule
\end{tabular}


==> files/tables/description.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
  &        &  count &        mean &        std &      min &         25\% &         50\% &         75\% &         max \\
State & Variable &        &             &            &          &             &             &             &             \\
\midrule
  & Gender &  256.0 &    0.589844 &   0.492825 &    0.000 &    0.000000 &    1.000000 &    1.000000 &    1.000000 \\
  & Age &  256.0 &   61.574219 &  12.110697 &   23.000 &   53.000000 &   60.000000 &   71.000000 &   91.000000 \\
  & State &  256.0 &    0.000000 &   0.000000 &    0.000 &    0.000000 &    0.000000 &    0.000000 &    0.000000 \\
  & Height &   75.0 &    1.706027 &   0.092245 &    1.473 &    1.625000 &    1.720000 &    1.770000 &    1.900000 \\
  & Weight &  251.0 &   96.159761 &  18.621362 &   55.300 &   83.700000 &   95.000000 &  107.000000 &  159.000000 \\
  & BMI &   66.0 &   33.887432 &   6.070832 &   21.660 &   29.890000 &   33.495000 &   36.980000 &   57.100000 \\
  & Diabetes &  256.0 &    1.281250 &   0.811075 &    0.000 &    1.000000 &    2.000000 &    2.000000 &    2.000000 \\
  & HbA1c/   mmol/mol &  202.0 &   61.376238 &  20.651986 &   37.000 &   45.000000 &   54.500000 &   71.000000 &  135.000000 \\
  & Gamma-G.T Level/   U/L &  137.0 &   78.664234 &  78.426181 &   14.000 &   35.000000 &   51.000000 &   95.000000 &  489.000000 \\
0  & Serum Cholesterol &  176.0 &    5.313693 &   1.302405 &    2.500 &    4.385000 &    5.200000 &    6.225000 &    9.300000 \\
  & HDL Cholesterol &  195.0 &    1.280256 &   0.421051 &    0.600 &    1.000000 &    1.200000 &    1.450000 &    3.500000 \\
  & Cholesterol Ratio &  157.0 &    4.304968 &   1.361320 &    1.200 &    3.000000 &    4.000000 &    5.000000 &    8.830000 \\
  & Triglyceride &  143.0 &    2.409650 &   1.445505 &    0.700 &    1.435000 &    2.000000 &    2.990000 &    7.910000 \\
  & Triglyceride/HDL Ratio &   80.0 &    2.203694 &   1.673170 &    0.400 &    1.087413 &    1.714407 &    2.753598 &    8.777778 \\
  & Systolic &  171.0 &  143.502924 &  15.476500 &  114.000 &  132.000000 &  142.000000 &  152.000000 &  223.000000 \\
  & Diastolic &  171.0 &   84.163743 &  10.320572 &   65.000 &   78.000000 &   80.000000 &   90.000000 &  122.000000 \\
  & TSH &   26.0 &    2.400000 &   1.398451 &    0.020 &    1.202500 &    2.375000 &    3.220000 &    5.050000 \\
  & T4 &   25.0 &   15.004000 &   2.793665 &    9.700 &   13.400000 &   14.500000 &   16.000000 &   22.900000 \\
  & HB &   22.0 &  145.136364 &   8.741229 &  123.000 &  140.250000 &  146.000000 &  150.500000 &  159.000000 \\
  & HMCT &   22.0 &    0.438636 &   0.026058 &    0.380 &    0.422500 &    0.440000 &    0.450000 &    0.500000 \\
  & months &  256.0 &    0.000000 &   0.000000 &    0.000 &    0.000000 &    0.000000 &    0.000000 &    0.000000 \\
  \midrule
  & Gender &  256.0 &    0.589844 &   0.492825 &    0.000 &    0.000000 &    1.000000 &    1.000000 &    1.000000 \\
  & Age &  256.0 &   61.574219 &  12.110697 &   23.000 &   53.000000 &   60.000000 &   71.000000 &   91.000000 \\
  & State &  256.0 &    1.000000 &   0.000000 &    1.000 &    1.000000 &    1.000000 &    1.000000 &    1.000000 \\
  & Height &   75.0 &    1.706027 &   0.092245 &    1.473 &    1.625000 &    1.720000 &    1.770000 &    1.900000 \\
  & Weight &  251.0 &   87.070120 &  17.351535 &   51.000 &   75.000000 &   84.400000 &   97.100000 &  140.000000 \\
  & BMI &   65.0 &   30.356462 &   5.922518 &   19.240 &   27.040000 &   29.270000 &   32.470000 &   53.620000 \\
  & Diabetes &  256.0 &    0.718750 &   0.867157 &    0.000 &    0.000000 &    0.000000 &    2.000000 &    2.000000 \\
  & HbA1c/   mmol/mol &  201.0 &   45.925373 &   9.318766 &   32.000 &   40.000000 &   43.000000 &   50.000000 &   84.000000 \\
  & Gamma-G.T Level/   U/L &  137.0 &   44.660584 &  39.049598 &    7.000 &   22.000000 &   32.000000 &   52.000000 &  260.000000 \\
1  & Serum Cholesterol &  174.0 &    4.892414 &   1.246772 &    2.400 &    4.025000 &    4.700000 &    5.700000 &    8.800000 \\
  & HDL Cholesterol &  189.0 &    1.412751 &   0.542463 &    0.700 &    1.090000 &    1.340000 &    1.610000 &    4.900000 \\
  & Cholesterol Ratio &  156.0 &    3.756667 &   1.073727 &    1.350 &    3.000000 &    3.775000 &    4.420000 &    7.000000 \\
  & Triglyceride &  132.0 &    1.522576 &   0.887664 &    0.560 &    0.930000 &    1.300000 &    1.795000 &    6.200000 \\
  & Triglyceride/HDL Ratio &   71.0 &    1.221976 &   0.935913 &    0.150 &    0.664018 &    0.963636 &    1.398688 &    5.777778 \\
  & Systolic &  170.0 &  132.100000 &  11.020503 &  108.000 &  125.000000 &  132.000000 &  139.500000 &  170.000000 \\
  & Diastolic &  170.0 &   77.794118 &   7.569713 &   54.000 &   71.250000 &   78.000000 &   82.000000 &  110.000000 \\
  & TSH &   26.0 &    1.919231 &   1.056757 &    0.140 &    0.855000 &    1.975000 &    2.720000 &    3.790000 \\
  & T4 &   25.0 &   15.480000 &   2.238675 &   11.400 &   13.900000 &   15.200000 &   16.200000 &   20.800000 \\
  & HB &   22.0 &  141.636364 &  10.513236 &  115.000 &  137.000000 &  142.000000 &  146.750000 &  161.000000 \\
  & HMCT &   22.0 &    0.421364 &   0.031517 &    0.330 &    0.410000 &    0.425000 &    0.440000 &    0.480000 \\
  & months &  256.0 &   22.199219 &  17.456370 &    1.000 &    8.000000 &   19.000000 &   32.000000 &   84.000000 \\
\bottomrule
\end{tabular}

